Down the Borel Hierarchy: Solving Muller Games via Safety Games

We transform a Muller game with n vertices into a safety game with (n!)^3 vertices whose solution allows to determine the winning regions of the Muller game and to compute a finite-state winning strategy for one player. This yields a novel antichain-based memory structure and a natural notion of permissive strategies for Muller games. Moreover, we generalize our construction by presenting a new type of game reduction from infinite games to safety games and show its applicability to several other winning conditions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{169}
\providecommand{\publicationstatus}{M. Faella, A. Murano (Eds.): Games, Automata, Logics\\
and Formal Verification (GandALF 2012)\\
EPTCS 96, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.96.13}{10.4204/EPTCS.96.13}}

